Coupled Rayleigh--Taylor and Faraday instabilities in vertically vibrated cylindrical containers

Interfacial instabilities govern the mixing in confined multiphase flows. Yet, the two mechanisms that drive them are usually studied independently: the pressure-gradient-driven Rayleigh--Taylor (RT) instability, which amplifies long-wavelength modes, and the parametrically forced Faraday instability, which selects shorter-wavelength harmonic or subharmonic modes. When an adverse density contrast and vertical vibration act together, the two compete, and neither alone describes the response. We use Floquet analysis to characterize the onset, growth, modal structure, and velocity fields of Faraday--RT waves in a vertically vibrated cylinder, resolved by azimuthal wavenumber, radial (Bessel) mode, and Floquet harmonic. The formulation recovers the classical RT and Faraday limits and reproduces the instability onset at the frequencies measured experimentally. For a free-sliding interface, increasing the vibration amplitude shifts the dominant instability mechanism from RT growth to subharmonic and then harmonic Faraday responses. Lateral confinement can also stabilize individual RT modes, which is not possible in an unbounded domain, although other Faraday modes may remain unstable. Pinning the contact line couples radial modes that otherwise evolve independently, allowing the unstable mode to be a superposition of RT-unstable and Faraday-stable components. This superposition alters the instability mechanism, producing a richer radial pattern. Reconstruction of the unstable modes shows the (linear) velocity fields that imaging cannot access and demonstrates how the instabilities can change the flow more broadly.

==> colors.tex <==
\definecolor{lightblue}{rgb}{0.63, 0.74, 0.78}
\definecolor{seagreen}{rgb}{0.18, 0.42, 0.41}
\definecolor{orange}{rgb}{0.85, 0.55, 0.13}
\definecolor{silver}{rgb}{0.69, 0.67, 0.66}
\definecolor{rust}{rgb}{0.72, 0.26, 0.06}
\definecolor{purp}{RGB}{68, 14, 156}

\colorlet{lightrust}{rust!50!white}
\colorlet{lightorange}{orange!25!white}
\colorlet{lightlightblue}{lightblue}
\colorlet{lightsilver}{silver!30!white}
\colorlet{darkorange}{orange!75!black}
\colorlet{darksilver}{silver!65!black}
\colorlet{darklightblue}{lightblue!65!black}
\colorlet{darkrust}{rust!85!black}
\colorlet{darkseagreen}{seagreen!85!black}

==> math_symbols.tex <==
\usepackage{bm}

\usepackage{xparse}
\DeclareDocumentCommand{\diff}{O{} m}{
	\frac{\mathrm{d} #1}{\mathrm{d}#2}
}
\DeclareDocumentCommand{\difftwo}{O{} m}{
	\frac{\mathrm{d}^2 #1}{\mathrm{d}#2^2}
}
\DeclareDocumentCommand{\pdiff}{O{} m}{
	\frac{\partial #1}{\partial #2}
}
\DeclareDocumentCommand{\pdifftwo}{O{} m}{
	\frac{\partial^{2} #1}{\partial #2^{2}}
}
\DeclareDocumentCommand{\integral}{O{} O{} m O{x}}{
	\int_{#1}^{#2} #3\ \mathrm{d}#4
}

\DeclareDocumentCommand{\bu}{}{\bm{u}}
\DeclareDocumentCommand{\bI}{}{\bm{I}}
\DeclareDocumentCommand{\bg}{}{\bm{g}}
\DeclareDocumentCommand{\bq}{}{\bm{q}}
\DeclareDocumentCommand{\bF}{}{\bm{F}}
\DeclareDocumentCommand{\bzeta}{}{\bm{\zeta}}

\DeclareMathOperator*{\argmin}{arg\,min} % thin space, limits underneath in displays

\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\At}{\mathrm{At}}

\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmi}{\mathrm{i}}
\DeclareMathOperator*{\argmax}{arg\!\max}
\newcommand{\transpose}{\mathsf{T}}

==> preamble.tex <==
\makeatletter
  \long\def\pprintMaketitle{\clearpage
  \iflongmktitle\if@twocolumn\let\columnwidth=\textwidth\fi\fi
  \resetTitleCounters
  \def\baselinestretch{1}%
  \printFirstPageNotes
  \begin{center}%
 \thispagestyle{pprintTitle}%
   \def\baselinestretch{1}%
    {\large\bf\@title}\par\vskip5pt
    \normalsize\elsauthors\par\vskip5pt
    \footnotesize\itshape\elsaddress\par\vskip10pt
    % \hrule\vskip12pt
    % \ifvoid\absbox\else\unvbox\absbox\par\vskip10pt\fi
    % \ifvoid\keybox\else\unvbox\keybox\par\vskip10pt\fi
    % \hrule\vskip12pt
    \end{center}%
  \gdef\thefootnote{\arabic{footnote}}%
  }
\makeatother

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\journal{}
\raggedbottom

% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }
% \raggedbottom

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{chngcntr}
\usepackage{abstract}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{epsf}
\usepackage{setspace}
\usepackage{soul}
\usepackage[margin=1in]{geometry}
\usepackage{booktabs}
\usepackage[version=4]{mhchem}
\usepackage{array} 
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{xcolor}
\usepackage{wrapfig}
\usepackage{physics}
\usepackage{multirow}
\usepackage[labelfont=bf,font=footnotesize]{caption}
\usepackage{subcaption}
% \usepackage{longtable}

\usepackage{tikz}

\usepackage{tabularx}
% \setlength\LTleft{0pt} 


\usepackage[]{siunitx}
\sisetup{
    separate-uncertainty = true,
    print-unity-mantissa=false,
    per-mode=symbol,
    range-phrase = \text{--}
}

\usepackage{setspace}
\setstretch{1.1}

\usepackage[]{microtype}

\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}

\input{colors.tex}

\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
}

\usepackage[nameinlink]{cleveref}
\crefname{equation}{}{}
% elsarticle bakes "Appendix" into the section number, so the aliased appendix
% name is left blank to avoid a doubled "Appendix Appendix" in \cref/\Cref.
% Names live here (global) so refs before \appendix resolve correctly; the
% per-label \crefalias tagging is applied at \appendix in main.tex.
\crefname{appendix}{}{}
\Crefname{appendix}{}{}
\usepackage{empheq}

\usepackage[parfill]{parskip}

\input{math_symbols.tex}

\bibliographystyle{bibsty.bst}

\newcommand{\baw}[1]{\textcolor{rust}{[[Ben says: #1]]}}
\newcommand{\shb}[1]{\textcolor{seagreen}{[[Spencer says: #1]]}}
\newcommand{\spencer}[1]{\textcolor{seagreen}{[[Spencer says: #1]]}}
\newcommand{\todo}[1]{\textcolor{red}{[[To-do: #1]]}}

